Presenting Profunctors

Motivated by problems in categorical database theory, we introduce and compare two notions of presentation for profunctors, uncurried and curried, which arise intuitively from thinking of profunctors either as functors C^op x D -> Set or C^op -> Set^D. Although the Cartesian closure of Cat means these two perspectives can be used interchangeably at the semantic level, a surprising amount of subtlety is revealed when looking through the lens of syntax. Indeed, we prove that finite uncurried presentations are strictly more expressive than finite curried presentations, hence the two notions do not induce the same class of finitely presentable profunctors. Moreover, an explicit construction for the composite of two curried presentations shows that the class of finitely curried presentable profunctors is closed under composition, in contrast with the larger class of finitely uncurried presentable profunctors, which is not. This shows that curried profunctor presentations are more appropriate for computational tasks that use profunctor composition. We package our results on curried profunctor presentations into a double equivalence from a syntactic double category into the double category of profunctors. Finally, we study the relationship between curried and uncurried presentations, leading to the introduction of curryable presentations. These constitute a subcategory of uncurried presentations which is equivalent to the category of curried presentations, therefore acting as a bridge between the two syntactic choices.

==> eptcsdata.tex <==
\providecommand{\firstpage}{88}
\providecommand{\publicationstatus}{D. Jaz Myers and M. Johnson (Eds.): International Conference\\
on Applied Category Theory 2024 (ACT 2024)\\
EPTCS 429, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.429.5}{10.4204/EPTCS.429.5}}
\pdfoutput=1

